Telelife: The Future of Remote Living

In recent years, everyday activities such as work and socialization have steadily shifted to more remote and virtual settings. With the COVID-19 pandemic, the switch from physical to virtual has been accelerated, which has substantially affected various aspects of our lives, including business, education, commerce, healthcare, and personal life. This rapid and large-scale switch from in-person to remote interactions has revealed that our current technologies lack functionality and are limited in their ability to recreate interpersonal interactions. To help address these limitations in the future, we introduce "Telelife," a vision for the near future that depicts the potential means to improve remote living better aligned with how we interact, live and work in the physical world. Telelife encompasses novel synergies of technologies and concepts such as digital twins, virtual prototyping, and attention and context-aware user interfaces with innovative hardware that can support ultrarealistic graphics, user state detection, and more. These ideas will guide the transformation of our daily lives and routines soon, targeting the year 2035. In addition, we identify opportunities across high-impact applications in domains related to this vision of Telelife. Along with a recent survey of relevant fields such as human-computer interaction, pervasive computing, and virtual reality, the directions outlined in this paper will guide future research on remote living.

==> 3_communication-tools.tex <==
\section{Current Practice}\label{sec:current_practice}
\kaan{To restructure this section as work, play and learn. And also add telecommunication tools section.}

This section outlines tools being used for 'telelife' that are currently in place today. We start with generic telecommunication tools that can be used in varies situations. We then describe tools that are dedicated to support remote work, learning and play.

\subsection{General tools for telecommunication}
Transmitting audio and video over the internet have enabled today's widespread applications such as video streaming, music streaming or teleconferencing. Transmission of voice over the internet similar to a telephone has been commercialized starting from mid-90s (i.e. VocalTec), which formed basis of Voice-over-Internet-Protocol (VoIP) of today.
In the meanwhile, transmitting videos over the internet has became a reality in parallel~\cite{tobagi1993starworks}.
As Real Time Streaming Protocol (RTSP)~\cite{schulzrinne1998real}, an application-level protocol for control over the delivery of data with real-time properties, is introduced, both audio and video transmission over the internet have been standardized.
Although teleconferencing, also known as video conferencing, has been experimented pre-internet age with telephone networks (i.e. Picturephone~\cite{dorros1971picturephone}), the teleconferencing tools relying on internet became widely available with the start of 2000s as RTSP is introduced (i.e. Skype).
\kiyoshi{Do we want to mention more early video conferencing tools?\\
- Apple CU-SeeMe in 1992\\
- Access Grid around the year 2000
}

Today's information-oriented distributed workers of the enterprises largely rely on these teleconferencing tools within their daily routines. In the meanwhile, the rest of the society becomes more familiar with teleconferencing with the COVID-19 pandemic situation. 

In this section, we survey a number of popular teleconferencing tools include FaceTime, Facebook Messenger, Microsoft Teams, Zoom, Gather.town, Skype, WhatsApp, LINE, and Google Meet, which we believe are the common and most popular tools for teleconferencing.
\subsection{Tools that support work}

\subsection{Tools that support learning}

\subsection{Tools that support play}




%\subsection{2D tools}\label{subsec:2d_tools}
%\kaan{}



\paragraph{User interface.}
The most used teleconferencing tools of our times are the 2D ones.
We believe that their popularity is due to their simplistic approach in representation with 2D, which allows usage without requiring any prior training or expertise.
All of the 2D teleconferencing tools that we have surveyed has a text based communication support, while also supporting video and audio communications.
The way that text, video or audio are arranged in their user interfaces is the major differentiation point among each other.
Common method in 2D UserInterfaces (UI) in teleconferencing is to tile views of participants on a screen, and to transmit audio from all participants to all the other in the teleconference.
This common method is followed by Facebook Messenger, Zoom, Gather.town, Skype, Whatsapp, and Google Meet with some differences in their tiling strategy in terms of number of participants visible to a single participant at one time.
FaceTime also follows the common method, however, offers an interesting variation in terms of tiling and highlighting participants, in which a participant's presentation is correlated with the audio levels of that participant, so basically more a participant speaks, more it becomes visible to the other participants in the UI.
An outlier and an interesting case, Gather.town use pixelated avatars to represent each participant in a 2D world. 
In Gather.town's UI, avatars can navigate in that 2D world with simple key presses on a keyboard.
A participant can only hear and see the others if that person is at a close proximity in this 2D world.
In this sense, Gather.town is an unique venue across 2D user interfaces as it introduces ``the hallway'' alike experiences~\cite{nakanishi2004freewalk}, where you can run into people like in the real life.
\huaishu{There are a huge amount of literature in the field of CSCW and CMC (computer-mediated communication) in terms of remote working. They are not from the technology perspective, but from social end. Not sure if we want to discuss this.}
\kaan{Huaishu will investigate on finding relevant parties from CSCW and CMC research.}

\paragraph{Hardware and software platforms.} 
Hardware and software platform required to have an access to these tools vary from case to case. 
For example, FaceTime requires a specific smartphone or a specific tablet brand, while WhatsApp, Skype, Facebook Messenger, Microsoft Teams can not only work with all smart devices with a dedicated application, they also provide access through a web browser. 
Therefore, they can also operate on personal computers and smart devices without the need of a dedicated application at all times.
On the other hand, Zoom can only work with a dedicated application both in the case of personal computers and smart devices.
Gather.town works on only on browsers, supporting both personal computers and smart devices.
All of these tools support text based messaging, and do not necessarily need a camera, a loudspeaker, and a microphone. 
However, these peripheral components are necessary to have a conversation with video and audio.
To our knowledge, there are no 2D teleconferencing tools that officially support VR/AR headsets or AR applications with smartphones.\huaishu{Not sure if the hardware/software platform is important to the survey. Also most of the software we mentioned here are fairly common and I would argue these platform information is kind of tacit knowledge.}
\kiyoshi{How about 2D-based VR systems? Mozilla Hubs / Cluster etc. that support both normal 2D UIs and VR headsets? How about virtual cameras like Snap Camera and VTuber systems? How about voice changers?}

\paragraph{Basic and novel features.}
Majority of the tools that we have surveyed provides a solution for file sharing instantly, which offers a productive approach to share documents, images, and videos.
Screen sharing is also common across all these tools to help participants at a call to be able to observe an another participant's screen.
All the teleconferencing tools offer a whiteboard for sketching by participants in a session.
Background replacement or blurring is also offered as a feature through add-ons in many cases. 
However, it should be noted that modern web cameras also offer such features in their driver software suite.
Microphone and loudspeaker levels can all be automatically adjusted by majority of these tools if a participants allow it.
To our knowledge, there is no add-on in any of these teleconferencing tools to remove the background audio or visual noise in the real-life surroundings of the participants.
Some of these software offers alive auto-captioning of conversations.
So far in our observation, gather.town is the only tool that offers spatial audio, which comes in handy when there are large numbers of participants. 
\kiyoshi{How about Remo and SpatialChat? }
This way, a participant in a gather.town session can hear users close by better than the ones at a distance.
Number of users supported in these tools vary from case to case, unpaid Zoom, Google Meet offers up to 100 participants in one session, while Microsoft Teams offer 250.
Paid versions of these tools offer a much higher number of participants up to 500 people in the case of Zoom.

\subsection{3D tools}\label{subsec:3d_tools} 
\jason{}
%\kiyoshi{What is the distinction between 2D and 3D?  What about a 3D (VR) tool on a desktop monitor? What about a head-tracked non-stereo system? What about 3DOF tracking not 6DOF?}

Originally, many 3D applications were run with a 2D UI on a 2D display. 
For example, Second Life \cite{zhu2007second} was a 3D application in which multiple users could log in, move throughout a vast 3D world, chat, and interact with the environment. 
The military also made significant progress in these areas in the 80's and 90's by building systems like SIMNET \cite{calvin1993simnet}, NPSNET \cite{macedonia1994npsnet}, DIVE \cite{carlsson1993dive} and BrickNet \cite{singh1994bricknet}, amongst others.
However, these applications still bound users by 2D screens, and direct eye contact or hand gestures were still not possible.

Fortunately, VR has now enhanced teleconferencing with 3D elements in a 3D display as a means for telecommunication, attracting a much larger user base. 
%\kaan{The use of VR supports multiple iterations of the same scene at different locations in the meantime, thus improves on sense of being at an another location.}
Over the past decade, a number of 3D tools have been put to use in various industries for the purposes of remote living, many with limited success. Applications like VRChat \cite{montemorano2020body} have been used for social gatherings, whereas applications like VRDesktop and Mozilla Hubs \cite{steed2020evaluating} have been used for academic conferences and research meetings. This section reviews the 3D tools that have been put into practice to date. 

Perhaps one of the first major tools to be used for remote socialization in 3D is the virtual world called Second Life, released in 2003. This application allows users to meet through an embodied avatar, and interactions happen in various areas of a social world, albeit via a 2D monitor at the time of release. Although research on multi-user virtual environments dates back to the 90's \cite{barrus1996locales}, the Second Life environment represented one of the first commercial releases of a 3D application that allowed for mass social gatherings and meetings.


While the application did not facilitate work functions like screen sharing or complex manipulations, it motivated a great deal of other work on 3D online spaces. From Second Life emerged a great deal of other 3D applications designed for more specific application areas. 


Another groundbreaking example was VR Desktop, an application released in 2016 that allowed users to stream their desktop into VR and work while completely immersed in a simulation (https://www.bigscreenvr.com/). This became a huge milestone for immersive work, being one of the first commercial applications to allow for immersive PC work. This kind of immersive environment was especially useful for programming VR eye tracking interfaces, as developers did not need to remove the display in order to develop, test, or debug code. Current versions of the software allow for multiple users, collaborative screen viewing, pointing, and emoting via controllers. 

Garau et al. emphasize the importance of realistic avatars, as this has a significant impact on gaze behavior. Consequently, the ability to live a productive remote life will be a function of how well VR interfaces can replicate or improve upon currently available technology.  


The work by Singh et al.~\cite{singh2020significant} on significant application of VR.\huaishu{I'm wondering if we also want to talk a bit of Spatial(https://spatial.io), which in a sense similar to VR Desktop, but really offer the co-located sharing experience and also tailored specifically to remote working with VR}

\subsubsection{Hardware}
\kiyoshi{}
Devices that people use. (be sure to cite relevant research). Predominantly: PCs, Tablets, Phones, Cameras, mics, etc. But not the ones that are not yet adopted.

2D stationary displays are widely used as a visual display for casual 3D tools. The rendering is done on the 3D data, and the result is displayed on a flat screen. However, the viewing angle of a typical desktop monitor is too small compared to the natural field of view of our human vision, to present, for example, a life-size conversation partner. Systems that use large monitors or multiple monitors (known as tiled display walls) to display body scale data have been introduced in some educational and research institutions, but are not widely used. In addition, binocular and motion parallax are not typically not provided so the reality of the presented content is limited.

3D (stereo) displays and stereo cameras or depth cameras are necessary for Telelife with binocular stereopsis. They are much more popular than before, but they are not yet common. Similarly, real-time viewpoint measurement and 3D acquisition, which are necessary for motion stereoscopy, are rapidly becoming available on smartphones, but they are not yet at the level that anyone can use. Therefore, typical video conferencing systems such as Zoom and Teams, for example, do not support binocular and motion parallax.

(more advanced but less common hardware follows)

\subsubsection{Software}
\paragraph{Teleconferencing.} 
The advent of virtual reality in the recent years has enabled 3D teleconferencing tools.

The work by Danielle Lottridge~\cite{lottridge2020insights} on videochat, and COVID-19.

WebXR~\kaan{Citation needed} toolkit has enabled many applications to support remote access through web for AR/VR device development.
% like the ones in the following: 
\jeeeun{}Similarly, there is a growing trend in moving workspace to online tools for creative design in 3D modeling, enabling anyone with modern web browsers can not only access design tools but also share and download design results using the cloud platforms.
SketchUp \cite{} has been beloved CAD tool for novices, to start their 3D modeling using graphical user interfaces.
One primary factor the SketchUp dragged the attention and excited users was its idea of online \emph{3D Warehouse}, which empowers non-experts to download sophisticated 3D models for interior design, gaming, and many more.
Many Autodesk design suites are popular in 3D modelers, that facilitate online sharing of design outcomes, such as TinkerCAD for beginners, and Fusion360 for advanced users \cite{}.
Designers create their 3D models throughout either online or local platforms
%\huaishu{Fusion 360 is mostly in local, tho it does support remote collaboration and online sharing}
, share the design for further customization by others using web link, import and rework based on co-designers' works.
Building and extending modular libraries of basic and/or advanced building blocks made asynchronous collaboration easier.
Regardless of the type of collaboration, sharing designs became critical for remote collaboration. Not only does it enable sharing of ideas and intermediate outcome between synchronous, more internal collaboration, but it also empowered idea for remix and recreation from the existing, similar to Github model that developers fork open API and recreate new opensource projects. 
A potential for asynchronous collaboration sparks  between non-inclusive group of people with lots of time and efforts so to reserve repetitive work.
Fast forwarded, On-shape is a recent addition with its full capability in running on cloud, supporting designing and synchronous team collaboration, project management via web browsers \cite{}
It removed needs to download and install complex software and run locally, and more importantly, more synchronous collaboration became possible at remote work places.
% \huaishu{https://www.onshape.com/en/, probably worth survey here, as it's purely web-based 3D modeling tool and is pretty much as powerful as fusion and support team collaboration - that partially solved cross-platform concern}
Yet, cross-platform collaboration and sharing have not been made any easier due to tool and design format compatibility, as well as different approaches in addressing creation environments.
% Taking the concern into our account and f
Further expanding the culture  of 'sharing' work results with the virtue, there have been also great advances in online open marketplaces for resource sharing, such as Thingiverse\cite{}, YouMagine\cite{}, GrabCAD\cite{}.
Blooming web culture made it possible for 3D models to be shared and reused between wider audiences cross platforms, elimiinating the needs to be equipped the domain specific knowledge for designs. 
% Fascinated by many inspiring designs that are exhibited through public platforms, casual users also started to design their own from scratch or by remixing others' designs, discuss the idea by commenting, share thoughts and earn knowledge for troubleshooting, which even contributed to the expansion of 3D printing online community for more asynchronous collaboration

% \huaishu{maybe also survey ipad/tablet based 3D modeling/sketching tools? For example Shapr3D is one popular paramedic design tool}

% \kiyoshi{Do we also want to mention 3D capture/reconstruction/photogrammetry tools? Many good ones are available for smartphones/tablets. }
Increasing use of online repository that contributes the democratization of open resources encouraged manufacturers and 3rd party partners to create 3D digital files of physical products, using advanced capture and reconstruction packages [ARCore, Photogrammetry, many more].
Recent advances in hardware such as LiDAR accelerates not only reconstruction but also real-time updates of real-world environments.

\subsection{Benefits and shortcomings}
All these introduced tools have impacted our lives in ways that we benefit, while they also bring their own shortcomings and disadvantages.
Here, we discuss about those benefits and shortcomings, accordingly.

\subsubsection{Benefits.}

Number of users of those 2D and 3D tools have seen a dramatic increase with the COVID-19 pandemic situation in 2019 and 2020. 
Those tools provided the users to freedom to get connected without having to follow a strict timeline like in the traditional work format (9 am to 5 pm), and enabled users to operate from any physical location that they like to be.

\paragraph{Work.}
As the real life physical events have been cancelled due to pandemic, virtualization of all these events with 2D and 3D teleconferencing tools has taken place.
Virtual conferences are not new and a small number of conferences have been successfully converted to virtual~\cite{leong2008surgeons}.
One major example is from a relevant scientific venue that chooses to use both 2D and 3D tools in parallel for the attendees, a premier conference on Virtual Reality (VR) organized by The Institute of Electrical and Electronics Engineers (IEEE).
IEEEVR has seen a dramatic increase in number of attendees from 500 in 2019 to 2000 in 2020.

\kiyoshi{
near 700 in 2018
over 1000 in 2019
over 2000 in 2020
}

The diversity among the attendees is also positively effected as attendees from countries that were previously less present were able to join.
This is due to factors such as reduced cost (i.e. cheaper registration, no travel or accommodation cost) and reduced or non-existing bureaucracy (VISA processes) in virtualization.
A similar trend has been observed in other venues (i.e. SIGCHI, SIGGRAPH or CVPR) as most of the events are replaced with a virtual version.

According to the survey by U.S. Travel association~\cite{eisinger2002meetings}, most of the cost of physical meetings and events is involved in travel related expenses, and those expenses can be as large as 327.3 billion USD per year in the U.S. alone.
Virtual conferences are believed to be removing all these costs from meetings and events.
As described by Kl\"{o}wer et al.~\cite{klower2020analysis}, the transport sector as a whole accounts for 24 percent of the annual global emissions of carbon dioxide.
Virtualization of professional events is expected to help reducing the global emissions caused by the transport.

\paragraph{Learning.}
Education arena has also seen a dramatic change as education events such as lectures, courses, workshops and tutorials all became online with the pandemic.
Many of these events are turned into a prerecorded format so that the attendees can follow these events in their own time and can replay the content again.
\misha{Misha's help here. She may be able to tell me more insights} 
Platforms such as Google Expeditions allow for students to virtually visit different historic places.  Teachers are able to conduct virtual field trips without leaving the classroom.  This provides for easy access for all students using technology as simple as smartphones and a cardboard frame \cite{siegle_seeing_2018}.  Other examples of using Virtual Reality Learning Environments (VRLE) for specialized training, such as surgical training and flight simulators, are also present.  VRLE can also take advantage of interactions with other systems and Internet of Things (IoT) devices \cite{valluripally_attack_2020}.

\paragraph{Play.}


\subsubsection{Shortcomings.}
As the number of users of these tools has increased, new shortcomings and disadvantages appeared as no tool is perfect in delivering the right experience for everyone in the society.
In the meanwhile, the requirements for each person using virtualization tools can be also very much personalized and conflicting with other people's requirements.

A major shortcoming observed in the virtual space is the balance in conversational fairness, where a person or a group of people can dominate a conversation, and this can lead to situation where certain people are suppressed or underrepresented.
To avoid such cases, in real life, moderators can help with turn taking and conversational balance for assuring fairness in important conversations by mediating in an unbiased way.
In the future, intelligent agents in virtual spaces can help with the turn taking and conversational balance in an improved way at every conversation if requested as those agents can have unlimited replicas running in parallel~\cite{rajan2016adaptive}.

As the number of interactions increases with the increasing usage of virtual spaces, users of those spaces started to mention term ``Zoom fatigue'' named after a common teleconferencing tool called Zoom, where too many virtual interactions causing feeling of tiredness or burn-out. 
This fatigue is believed to be due to lack of natural social cues in virtual spaces.
For example, a typical virtual space for teleconferencing requires a level of focus, where you need to have a face to face conversations with all the participants at once.
This is burdensome for the majority of the users, and in many cases requires focus of the users to be at the teleconference at all times.
The work by Fosslien and Duffy~\cite{fosslien2020combat} expresses that combating ``Zoom fatigue'' is possible by avoiding multitasking in virtual spaces, planning on breaks in between virtual meetings, intentionally reducing the onscreen stimuli such as user backgrounds or self view, making virtual social events as opt-in, and switching to phone calls or emails for some of the meetings.

The habits of users in terms of sharing also effect the outcome of the events just like in the real life.
As most of the users of a virtual space leaving their cameras off or audios off, it will simply lead to less participation, therefore decreasing the effectiveness of virtual spaces for work, play and learn.

Virtual events that has participants around the world deals with the challenge of identifying a timezone convenient for all the participants.
To our knowledge, overcoming limitations related to holding a synchronous event across different timezones is an open challenge that has no solution 


\huaishu{Accessibility might not be the focus, but that is definitely one short comings here, that with all the new platforms, how to promote or guarantee equal access for all }
\misha{Probably Misha}\huaishu{ or Huaishu can help here.}

\jeeeun{Should we talk about Tool/format compatibility here?}

\paragraph{Work.}


\paragraph{Education.}
We expect this type of shift to positively influence the education in the long timeframe, however it also poses a personalized challenge for students to have higher levels of self determination in following the content. 
Like the other use cases, people has turned into collaborative settings to avoid lack of motivation, and this is mostly done by meeting on a virtual platform that mimics a virtual coffee shop, where people are surrounded with other people while they are working.

